Adinkras and Pure Spinors

The nilpotence variety for extended supersymmetric quantum mechanics is a cone over a quadric in projective space. The pure spinor correspondence, which relates the description of off-shell supermultiplets to the classification of modules over the corresponding hypersurface ring, reduces to a classical problem of linear algebra. Spinor bundles, which correspond to maximal Cohen-Macaulay modules, serve as basic building blocks. Koszul duality appears as a deformed version of the Bernstein-Gel'fand-Gel'fand correspondence that we make fully concrete. We illustrate in numerous examples the close relationship between these connections and the powerful graphical technology of Adinkras, which appear as a decategorification of special complexes on quadrics. We emphasize the role of R-symmetry for recovering higher-dimensional gauge and gravity multiplets.

==> S7outlook.tex <==
\section{Outlook}
\label{sec:outlook}

Koszul duality provides an equivalence between the derived categories of modules over $\mbox{\sffamily{D}}^\flat (A\mbox{-\sffamily{Mod}})$ and $\mbox{\sffamily{D}}^\flat (A^!\mbox{-\sffamily{Mod}})$.  One might be afraid that this simply exchanges one difficult problem for another.  The universal enveloping algebra $U_{\mathbf{k}} (\mathfrak{t}^{d,N})$ of the supertranslation algebra is an associative but non-commutative algebra, while its Koszul dual --- the ring of functions over the nilpotence variety is commutative.  This offers some hope.  Similar to the Borel--Weil--Bott theorem, the powerful geometric technique of Kempf--Lascoux--Weyman produces syzygies from desingularizations of vector bundles over projective spaces \cite{Weyman03}.  Ultimately, it appeals to Grothendieck duality \footnote{For a modern introduction, see \cite{Neeman20}.}.  
 
A beautiful introduction to this set of ideas is in \cite{Sam16}, which goes on to produce representations of the orthosymplectic group using modules over the corresponding nilpotence variety.  In a special case, this produces representations of the 6d $(N, 0)$ supertranslation algebras that lift to the superconformal algebra.  This can be seen as a far-reaching generalization of the classical Buchsbaum–Rim complex used to produce the BV complex for the 6d (1,0) hypermultiplet in \cite{Eager22}.

The 6d $N=1$ hyper-multiplet has an off-shell BV description that respects both the 6d Lorentz and $SU(2)$ R-symmetry.  It can be used to construct a supersymmetric sigma model in six-dimensions.  The hypermultiplet reduces to the $(4,8,4)$ $N=8$ multiplet in one-dimension with $SO(5)$ R-symmetry.  This R-symmetry realizes Verbitsky's $SO(5,1)$ action on the cohomology of hyperK\"ahler manifolds \cite{Figueroa97}.  The reduction and twist of the theory from 6d to 3d results in Rozansky--Witten theory.  Formally, it shares many similarities with ordinary Chern--Simons theory.  Motivated by this, it would be interesting to use the multiplets constructed, to consider supersymmetric quantum mechanics on moduli spaces of generalized instantons and to define K-theoretic enumerative invariants.

A fruitful way to generate supersymmetric quantum mechanics on generalized instanton moduli space is by dimensionally reducing topologically twisted gauge theories on $X \times S^1$ to $S^1$ \cite{Baulieu98}.  This often arises in the study of branes, and the prototypical example is the quiver quantum mechanics description of the ADHM moduli space arising from the D0-D4 system.

Generalized enumerative invariants are expected to be summed in twisted supergravity.  The membrane index is defined on eleven-dimensional supergravity backgrounds of the form $Z \times S^1$ where $Z$ is a Calabi--Yau five-fold with a $ \mathbb{C}^{\times}$ action.  The M-theory index of $Z$ is conjectured to be related to a certain K-theoretic Donaldson-Thomas invariants of threefolds $X$ that arise as fixed points of the $\mathbb{C}^{\times}$ action \cite{Nekrasov16}.  The membrane index is computed in twisted supergravity in \cite{Raghavendran11d} and is closely related to the superconformal index \cite{SCIM2}.   A new proposals for relating the algebra of $G_2$-instantons to twisted M-theory \cite{CostelloMtheory, Eager11d, Hahner11d} was made in \cite{DelZotto21}.

Similarly reducing theories from $X \times T^2$ to $T^2$ results in elliptic invariants.  It would be interesting to derive elliptic analogs of family Donaldson--Witten invariants by reducing BCOV theory coupled to holomorphic Chern--Simons theory, simplifying the derivation of \cite{Cushing:2023rha}.

We hope that the systematic study of the pure spinor formalism and adinkras with $R$-symmetry will help in aid of the grand challenge of \cite{GatesChallenge}.

==> hacks.tex <==

\makeatletter

%%%
%%%%%% draftcontrol
%%%%%%

\expandafter\ifx\csname draftcontrol\endcsname\relax\global\def\draftcontrol{0} 
\fi 

{\count255=\time\divide\count255 by 60 
\xdef\hourmin{\number\count255} 
\multiply\count255 by-60\advance\count255 by\time 
\xdef\hourmin{\hourmin:\ifnum\count255<10 0\fi\the\count255}} 
\def\draftdate{\number\month/\number\day/\number\year\ \ \ \hourmin } 

\def\@version#1{%
  \ifnum\draftcontrol=1 
  \typeout{}\typeout{#1}\typeout{} 
  \vskip3mm\centerline{%
    \hbox{%
      \fbox{\normalsize{\tt DRAFT -- #1 -- }%
          {\draftdate}}}}\vskip3mm 
\fi} 
\let\version\@version 

%%% 
%%%%%% titlepage (adapted from article.cls)
%%%%%%%%%

\newcommand\makepapertitle{\par
  \begingroup 
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}% 
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}% 
    \long\def\@makefntext##1{\parindent 1em\noindent 
            \hb@xt@1.8em{% 
                \hss\@textsuperscript{\normalfont\@thefnmark}}##1}% 
     \newpage 
     \global\@topnum\z@   % Prevents figures from going at top of page. 
     \@makepapertitle 
     \thispagestyle{empty}\@thanks 
  \endgroup 
  \setcounter{footnote}{0}% 
  \global\let\thanks\relax 
  \global\let\makepapertitle\relax 
  \global\let\@makepapertitle\relax 
  \global\let\@thanks\@empty 
  \global\let\@author\@empty 
  \global\let\@date\@empty 
  \global\let\@title\@empty 
  \global\let\title\relax 
  \global\let\author\relax 
  \global\let\date\relax 
  \global\let\and\relax 
  % \def\version{\let\version\@version\@gobble} 
  }
\def\@makepapertitle{% 
  \newpage 
   \ifnum\draftcontrol=1 {} 
   \version\versionno 
   \vskip 5.5em% 
   \else 
   \hfill\hbox to 3cm {\parbox{5.5cm}{\@pubnum}\hss}% 
   \vskip 3.5em% 
   \fi 
   \begin{center}% 
   \let \footnote \thanks 
      {\hskip -0\textwidth \hbox to 1\textwidth% 
        {\centerline{\Large\bf{\noindent%
	\parbox[t]{1.3\textwidth}{\begin{center}\@title\end{center}}}}}}% 
     \vskip 1.2em% 
     {\normalsize%\large 
       \lineskip .5em% 
       \begin{tabular}[t]{c}% 
         \@author 
       \end{tabular}\par}% 
     \vskip 1.5em% 
     {\@bstract}% 
     \end{center}% 
     \vfill
     \@date%
     \vskip 1.5em%
    \noindent
    \rule{12em}{.02em}\par\noindent
    \@email%
   \par 
} 

\gdef\@pubnum{} 
\def\pubnum#1{% 
  \gdef\@pubnum{#1}} 

\gdef\@bstract{} 
\def\Abstract#1{% 
  \gdef\@bstract{% 
   \parbox{\textwidth-0pc}{% 
   \centerline{\bf Abstract}\penalty1000 
   \noindent%\abstractfont \baselineskip=12pt 
   \renewcommand\baselinestretch{1.0} 
   {#1}}} 
} 

\gdef\@email{}
\def\email#1{%
   \gdef\@email{%
   Email: {\tt #1}}
}

%%%
%%%%%% Table of contents
%%%%%%%%%

\setcounter{tocdepth}{2}
\renewcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{.5em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\renewcommand*\l@subsection{\addvspace{.0em \@plus\p@}\@dottedtocline{2}{1.5em}{2.3em}}
\renewcommand*\l@subsubsection{\addvspace{-.2em \@plus\p@}\@dottedtocline{3}{3.8em}{3.2em}}

%%% 
%%%%%% pagestyle 
%%%%%%%%%  

\def\ps@paper{\let\@mkboth\@gobbletwo% 
     \ifnum\draftcontrol=1 
        \def\@oddfoot{\hbox to \textwidth{\tiny \versionno \hfil\tiny\draftdate}% 
        \hskip -\textwidth \hbox to \textwidth{\hfil\rm\thepage\hfil}}% 
     \else\def\@oddfoot{\hbox to \textwidth{\hfil\rm\thepage\hfil}} 
     \fi 
     \let\@evenfoot\@oddfoot 
} 

%%%
%%%%%% Bibliography
%%%%%%%%%

%%% this saves a bit of space
\renewcommand*{\bibsetup}{%
  \interlinepenalty=5000\relax
  \widowpenalty=10000\relax
  \clubpenalty=10000\relax
  \raggedbottom
  \frenchspacing
  \biburlsetup
  \renewcommand\baselinestretch{1.1}
}
\renewcommand{\bibfont}{\normalfont\small}
\setlength\bibitemsep{0.2em}
\setlength\bibhang{1em}

%%% this suppresses the In: 
\renewbibmacro{in:}{}
\DeclareFieldFormat{doilink}{%
  \iffieldundef{doi}%
  {#1}%
  {\href{https://doi.org/\thefield{doi}}{#1}}
}
%%% and puts doi link around journal reference
%%% (hacked from standard.bbx https://ctan.org/tex-archive/macros/latex/contrib/biblatex/latex/bbx?lang=en)
\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \setunit{\printdelim{nametitledelim}}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{bytranslator+others}%
  \newunit\newblock
  \printfield{version}%
  \newunit\newblock
  \usebibmacro{in:}
  \iffieldundef{journaltitle}
   {\printtext[journaltitle]{Preprint} \mkbibparens{\printdate}}
   {\printtext[doilink]{%
    \usebibmacro{journal+issuetitle}%
    \newunit
    \usebibmacro{byeditor+others}%
    \newunit
    \usebibmacro{note+pages}%
    \newunit\newblock
    \iftoggle{bbx:isbn}
      {\printfield{issn}}
      {}%
   }
   }
  \newunit\newblock
  \usebibmacro{doi+eprint+url}
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
    {\usebibmacro{related:init}%
     \usebibmacro{related}}
    {}%
  \usebibmacro{finentry}}

%%% this puts brackets around arxiv if journal exists
\letbibmacro{nakedEprint}{eprint}
\renewbibmacro*{eprint}{%
  \iffieldundef{eprint}
    {}
    {\iffieldundef{journaltitle}
      {\usebibmacro{nakedEprint}}
      {\printtext{{\usebibmacro{nakedEprint}}}}} %\mkbibbrackets I think there are too many brackets
}
%%% and changes format of [eprint:arxiv]
%%% (hacked from: https://packages.oth-regensburg.de/ctan/macros/latex/contrib/biblatex/latex/biblatex.def)
\DeclareFieldFormat{eprint:arxiv}{%
  \ifhyperref
    {\href{https://arxiv.org/\abx@arxivpath/#1}{%
       \nolinkurl{arXiv:#1}%
       \iffieldundef{eprintclass}
         {}
         {\addspace{\mkbibbrackets{\thefield{eprintclass}}}}}}  %%% remmoved \texttt
    {\nolinkurl{arXiv:#1}%
     \iffieldundef{eprintclass}
       {}
       {\addspace{\mkbibbrackets{\thefield{eprintclass}}}}}}   %%% removed \texttt

\makeatother
